Electric Double Layer from Phase Demixing Reinforced by Strong Coupling Electrostatics

Ionic liquids (ILs) are appealing electrolytes for their favorable physicochemical properties. However, despite their longstanding use, understanding the capacitive behavior of ILs remains challenging. This is largely due to the formation of a non-conventional electric double layer (EDL) at the electrode-electrolyte interface. This study shows that the short-range Yukawa interactions, representing the large anisotropically charged ILs, demix IL to create a spontaneous surface charge separation, which is reinforced by the strongly coupled charge interaction. The properties of the condensed layer, the onset of charge separation, and the rise of overscreening and crowding critically depend on the asymmetry of Yukawa interactions.

==> texFiles/00_abs.tex <==
\begin{abstract}
Ionic liquids (ILs) are appealing electrolytes for their favorable physicochemical properties. However, despite their longstanding use, understanding the capacitive behavior of ILs remains a challenge. This is largely due to the formation of a non-conventional electric double layer (EDL) at the electrode-electrolyte interface. Phenomenological theories proposed that the IL EDL could be enhanced by ion-ion correlation. In this study, we show that the combination of the long-range Coulomb and the short-range Yukawa interactions induce the IL EDL even at low surface charge densities. 
The demixing of IL due to Yukawa interaction at the surface enhances the development of condensation layer. 
It is observed that the structure of EDLs strongly depends on the asymmetry of Yukawa interactions. 
We also discuss the onset of charge separation and the relation between overscreening and crowding.
\end{abstract}

==> texFiles/01_intro.tex <==
\section{Introduction}
Room-temperature ionic liquids (RTILs) are combinations of large organic cations and organic, inorganic anions with delocalized charges. This prevents them from forming crystalline structures at room temperatures, unlike conventional inorganic salts~\cite{IL1, IL2, screen}. Due to these extraordinary features, RTILs offer several advantages for energy storage applications, such as low volatility, good solvent properties, high thermal stability, and environmental sustainability~\cite{adv1, adv2, application1, application2, application3, application4}, which are especially fit for future energy storage devices, supercapacitors, or ultracapacitors.
Especially, some essential features for high-technology devices (\textit{e.g.} wireless devices and electric cars), such as higher-rate energy harvesting and long-lasting supercapacitance are related to the electric double layer (EDL) structures in RTILs~\cite{supercapacitor1, supercapacitor2, supercapacitor3, supercapacitor4, supercapacitor5}. 
While conventional point charge models predict the development of condensation layer at very large surface charge density, IL exhibits EDL at very low surface charge density, and even overscreening and crowding which are very difficult to achieve without the presence of the multivalent counterions within the point charge models. 
The key differences are from the large and structured IL molecules and their delocalized charges. 
It is challenging to understand how to embody these properties to the microscopic mechanism, and crucial in utilizing ILs for energy device applications. ~\cite{orland3, ic1, ic2, ic3}. 

Bazant, Storey, and Korneyshev (BSK)~\cite{bsk} are among the first to incorporate a short-range electrostatic correlation to the EDL. They showed that a phenomenological modification of the Poisson equation with an extra fourth-order potential gradient term, reflecting a short-range electrostatic correlation, explains the divergence of differential capacitance, may be triggered by overscreening. They further asserted that crowding beats overscreening at higher external fields. 

Since the phenomenological description of BSK model, efforts to uncover the microscopic mechanism for unconventional EDL features have been made. 
D\'{e}mery \textit{et al.} solved 1D lattice Coulomb gas (1D LCG) under the constant voltage ensemble. 
Their solvable one-dimensional model showed that the 1D LCG undergoes a first-order phase transition dense phase and dilute phase by adjusting fugacity~\cite{1d1, 1d2}. They claimed that the transition is closely related to the discontinuous jump in differential capacitance and the transition between camel- and bell-shape capacitance.

Other directions of the approaches use statistical field theory for charged many-body. Earlier mobile point charges with fixed macro-ions were treated within the framework of the statistical field theory of ion systems~\cite{coalson1, coalson2, orland1, orland2, orland3}. 
These works consider the condensed layer as a boundary condition and focus on the bulk electrostatics at the saddle point.
Recently, Bossa et al. adopted the free energy analysis approaches incorporating Yukawa potential to consider the symmetric steric term and successfully reproduced the fourth order potential gradient in BSK equation~\cite{bossa, coulyukawa}. They showed that the interplay between short-ranged Yukawa and long-ranged Coulomb interactions can lead to the instability of ILs near an electrode. This instability is characterized by a divergent differential capacitance, indicating a first-order transition~\cite{bossa}.

In this work, we present the microscopic origin of the unconventional EDL formation and consequent phase transition of RTIL capacitance starting from the statistical field theory. 
We have derived free energy functionals for asymmetric ionic liquids and obtained the modified Poisson equations using saddle point approximation. We investigate the phase transition triggered by the interplay of the asymmetric short-range correlation and the electrostatic interaction. We verify the theoretical results by comparing molecular dynamics simulations. Furthermore, we present the effect of the external field to the phase behavior. Our work on room-temperature ionic liquids (RTILs), can extended to the various systems~\cite{various1, various2, various3, various4}.

==> texFiles/02_theory_methods.tex <==
\section{Model}
\subsection{Statistical Field Theory}
We develop a lattice based model for electrode of surface charge density $\sigma_{e}$ at $x=0$. The number of the particle at $r$ is $n_{\pm}(r)$ and $\sum_r n_{\pm} = N_{\pm}$. The local densities of each species are $\rho_{\pm}(r)=n_{\pm}(r)/\nu$, where $\nu$ is the volume of each lattice. The local charge density is defined as $\rho_{c}(r)=\rho_{+}(r) - \rho_{-}(r)$. 

Particles interact each other through Coulombic and Yukawa interaction:
\begin{equation}
\begin{split}
    \beta u_{+,+} &= \frac{l_{B}}{r} + a \frac{e^{-\kappa r}}{r} \\
    \beta u_{+,-} &= -\frac{l_{B}}{r} + c \frac{e^{-\kappa r}}{r} \\
    \beta u_{-,-} &= \frac{l_{B}}{r} + b \frac{e^{-\kappa r}}{r},
\end{split}\label{eq:interaction}
\end{equation}
where $l_{B}$ is the Bjerrum length, and $a, b$ and $c$ are the Yukawa interaction parameters, and $\beta=k_{B}T$. Then, the total interaction potential energy is represented by 
\begin{equation}
\begin{split}
    \beta\mathcal{U}_{tot} &= \frac{1}{2}\int{drdr'\rho_{c}(r)v_{c}(r-r')\rho_{c}(r')}\\ 
    &+ \frac{1}{2}\int{drdr'\begin{pmatrix}\rho_{+}(r)\\ \rho_{-}(r)\end{pmatrix}^{T}A_{h}v_{y}(r-r')\begin{pmatrix}\rho_{+}(r)\\ \rho_{-}(r)\end{pmatrix}},
\end{split}
\end{equation}\label{eq:total1}
where $A_{h} = \begin{pmatrix} a & c \\ c & b\end{pmatrix}$, $v_{c}(r) = l_{B}/r$, and $ v_{y}(r) = e^{-\kappa r}/r$. Similarity transformation decouples the Yukawa term with eigenstates,
\begin{equation}
    \begin{split}
        \beta\mathcal{U}_{tot} &= \frac{1}{2}\int{drdr'\rho_{c}(r)v_{c}(r-r')\rho_{c}(r')} \\
                          &+ \frac{1}{2}\int{drdr'\rho_{1}(r)v_{y,1}(r-r')\rho_{1}(r')} \\
                          &+ \frac{1}{2}\int{drdr'\rho_{2}(r)v_{y,2}(r-r')\rho_{2}(r')},
    \end{split}
\end{equation}\label{eq:total2}
where $v_{y,i}(r) = \lambda_{i}v_{y}(r)$ for $i=1,2$. The $\lambda_{i}$ is
\begin{equation*}
    \begin{split}
        \lambda_{1}&=a\cos^{2}\theta+2c\sin\theta\cos\theta+b\sin^{2}\theta \\ 
        \lambda_{2}&=a\sin^{2}\theta-2c\sin\theta\cos\theta+b\cos^{2}\theta,
    \end{split}
\end{equation*}
and $\rho_{i}(r)$ is
\begin{equation*}
    \begin{split}
        \rho_{1}(r)&=\rho_{+}(r)\cos\theta+\rho_{-}(r)\sin\theta \\
        \rho_{2}(r)&=-\rho_{+}(r)\sin\theta+\rho_{-}(r)\cos\theta.
    \end{split}
\end{equation*}
Here, $\theta$ satisfies, 
\begin{equation*}
    \tan 2\theta = \frac{2c}{a-b}.
\end{equation*}

The canonical partition function of the system is,
\begin{equation}
    \begin{split}
    \mathcal{Z}_{c} &= \sum\limits_{\{n_{\pm}(r)\}}\delta\left(\sum_{r}n_{+}(r)-N_{+}\right)\delta\left(\sum_{r}n_{-}(r)-N_{-}\right)e^{-\mathcal{U}_{tot}} \\
    &=\sum_{\{n_{\pm}(r)\}}
    \delta\left(\sum_{r}n_{+}(r)-N_{+}\right)
    \delta\left(\sum_{r}n_{-}(r)-N_{-}\right) \\
    &\times\exp\left(-\frac{1}{2}\int{drdr'\rho_{c}(r)v_{c}(r-r')\rho_{c}(r')}\right. \\
    &\left.\quad\quad\quad\,\,-\frac{1}{2}\int{drdr'\rho_{1}(r)v_{y,1}(r-r')\rho_{2}(r')}\right. \\
    &\left.\quad\quad\quad\,\,-\frac{1}{2}\int{drdr'\rho_{1}(r)v_{y,2}(r-r')\rho_{2}(r')}\right).
    \end{split}
    \label{eq:canonical}
\end{equation}

It is more practical to deal with the grand canonical ensemble, 
\begin{equation*}
\begin{split}
\mathcal{Z_{\lambda}}=\sum_{N_{+}=0}^{\infty}\sum_{N_{-}=0}^{\infty}
\frac{\lambda_{+}^{N_{+}}}{N_{+}!}\frac{\lambda_{-}^{N_{-}}}{N_{-}!}\mathcal{Z}_{c}.
\end{split}
\end{equation*}
where fugacities $\lambda_{\pm}$ are function of the chemical potential $\mu_{\pm}$, $\lambda_{\pm} = e^{\mu_{\pm}}$.

The Hubbard-Stratonovich transformations setting $\lambda_{\pm}=\lambda_{s}$ for the charge neutrality condition yields,
\begin{align}
\mathcal{Z}_{\lambda} &= \int \mathcal{D}\phi_{e}\mathcal{D}\phi_{1}\mathcal{D}\phi_{2} \exp\left(-\frac{1}{8\pi l_{B}}\int dr \left(\nabla\phi_{e}\right)^{2} \right. \nonumber \\
    &\left. -\frac{1}{8\pi\lambda_{1}}\int dr \left(\left(\nabla\phi_{1}\right)^{2} + \kappa^{2}\phi_{1}^{2}\right)\right. \nonumber \\
    &\left. -\frac{1}{8\pi\lambda_{2}}\int dr \left(\left(\nabla\phi_{2}\right)^{2} + \kappa^{2}\phi_{2}^{2}\right)\right) \label{eq:gandcanonical2} \\ 
    &\times \exp\left(\frac{1}{\nu}\int dr \ln{\left(\lambda_{s}\left(\textbf{e}_{1}+\textbf{e}_{2}\right)\right)}\right) \nonumber,
\end{align}
where $\textbf{e}_{1} = \exp\left(-i\phi_{e}-i\phi_{1}\cos\theta+i\phi_{2}\sin\theta\right)$ and $\textbf{e}_{2} = \exp\left(+i\phi_{e}-i\phi_{1}\sin\theta-i\phi_{2}\cos\theta\right)$. The free energy is,
\begin{equation}
\begin{split}
    \beta\mathcal{F} = &\int dr\left[-\frac{1}{8\pi l_{B}}\left(\nabla\psi_{e}\right)^{2} -\frac{1}{8\pi\lambda_{1}}\left\{\left(\nabla \psi_{1}\right)^{2}+\kappa^{2}\psi_{1}^{2}\right\}\right. \\
    &\left.-\frac{1}{8\pi\lambda_{2}}\left\{\left(\nabla \psi_{2}\right)^{2}+\kappa^{2}\psi_{2}^{2}\right\}\right] + \eta\left(\tilde{\textbf{e}}_{1}, \tilde{\textbf{e}}_{2}\right),
\end{split}
\end{equation}
where 
\begin{equation*}
    \eta\left(\tilde{\textbf{e}}_{1}, \tilde{\textbf{e}}_{2}\right) = -\frac{1}{\nu}\int dr \ln\left\{\lambda_{s}\left(\tilde{\textbf{e}}_{1} + \tilde{\textbf{e}}_{2}\right)\right\},
\end{equation*}
and $\tilde{\textbf{e}}_{1} = \exp\left(-\psi_{e}-\psi_{1}\cos\theta+\psi_{2}\sin\theta\right)$ and $\tilde{\textbf{e}}_{2} = \exp\left(+\psi_{e}-\psi_{1}\sin\theta-\psi_{2}\cos\theta\right)$.
The functional integral is approximated by the saddle-point field, 
\begin{equation}
\begin{split}
    &\frac{1}{4\pi l_{B}}\nabla^{2}\psi_{e} = \frac{1}{\nu} \frac{\tilde{\textbf{e}}_{2}-\tilde{\textbf{e}}_{1}}{\tilde{\textbf{e}}_{1}+\tilde{\textbf{e}}_{2}} \\ \\
    &\frac{1}{4\pi \lambda_{1}}\left(\nabla^{2}-\kappa^{2}\right)\psi_{1} = \frac{1}{\nu} \frac{-\cos\theta\tilde{\textbf{e}}_{1} - \sin\theta\tilde{\textbf{e}}_{2}}{\tilde{\textbf{e}}_{1}+\tilde{\textbf{e}}_{2}} \\ \\
    &\frac{1}{4\pi \lambda_{2}}\left(\nabla^{2}-\kappa^{2}\right)\psi_{2} = \frac{1}{\nu} \frac{\sin\theta\tilde{\textbf{e}}_{1} - \cos\theta\tilde{\textbf{e}}_{2}}{\tilde{\textbf{e}}_{1}+\tilde{\textbf{e}}_{2}}.
\end{split}\label{eq:mf}
\end{equation}

If $a=b=c$, there is neither asymmetry nor phase demixing contribution, and hence the electrostatic case is recovered. Overcharging or crowding is not recovered in this mean-field electrostatic regime. 
If $a-b \gg c$, then $\theta \simeq 0$. $\lambda_1 = a, \lambda_2 = b$. $e_1 = \exp\left\{-\psi_e-\psi_1 \right\}, e_2 = \exp\left\{\psi_e-\psi_2 \right\}$. $\frac{e_1}{e_1+e_2} = \frac{1}{1+\exp\left\{2\psi_e-\psi_2+\psi_1\right\}}$ and $\frac{e_2}{e_1+e_2} = \frac{1}{1+\exp\left\{-2\psi_e+\psi_2-\psi_1\right\}}$.


\subsection{Molecular Dynamics Simulation}
Based on Benjamin's coarse-grained model, which successfully induced the divergence of differential capacitance~\cite{benjamine}, Yukawa interaction is added to compare the results with the theory. 
Cations and anions carry charges at their center. As the reference work claimed, image charge interactions are included to study the divergence of differential capacitance. In addition to the long-range Coulomb interaction, particles interact each other through combined short-ranged pair potentials. All input parameters and output quantities are scaled by fundamental quantities. The main dimensionless physical quantities are provided in section A of Supporting Information.
Simulations are performed using the LAMMPS in the canonical ensemble~\cite{lammps}. The system consists of $1000$ real particles and $1000$ image particles, with a number density of $\rho=0.8$, and the temperature is set to $T=1$ using Langevin thermostat. The simulation box is created with the size of $2L \times L \times L$ where the value of $L$ is determined to satisfy the desired number density $\rho=N/V$. Furthermore, wall potentials are applied at $x=0$ and $x=L$ to represent two smooth planar electrodes. The relative permittivity, $\epsilon_{r}$, and Bjerrum length, $l_{B}$, are set to typical values used for RTIL systems~\cite{Kornyshev, bsk, wakai}, \textit{i.e.}, $\epsilon_{r}=12$ and $l_{B}=10$. Moreover, the elementary charges have reduced magnitudes of $q=\sqrt{\epsilon_{r} l_{B} T} \simeq 11$.

Energy minimization and equilibration are performed for each simulation over $10^{5}$ timesteps with a step size $\tau=0.001$. Another $3\times10^{6} \tau$ steps are spent for data production. As Benjamin \textit{et al.} claimed simulation converges to the equilibrium state regardless of the initial configurations~\cite{benjamine}.

In EDLCs simulations, it is crucial to properly treat the interactions between ions and electrodes. An image charge method is an effective way to embrace the dielectric discontinuity between the electrolyte and the surrounding medium. When the relative permittivity of the bounding material is lower (higher) than that of the electrolyte, ions experience repulsion (attraction) with their images. 
The image charge method is implemented in LAMMPS by Dwelle and Willard~\cite{image_charge}. It is based on the method proposed by Hautman \textit{et al.}, which involves considering infinitely repeating systems of image charges when simulating a three-dimensional system with ions~\cite{rhee}. The simulation system is divided into two subsystems: a real system on the right side ($0 < x < L_{x} )$ and an image system on the left side $( -L_{x} < x < 0 )$. The image particles possess charges opposite to those of the real particles in the real system, and they are generated at positions symmetric to the real particles relative to the electrode located at $x=0$. The whole simulation box is repeated as a unit cell.

The short-range ion-ion correlation is modeled by shifted Yukawa potential. For here the potential has the form
\begin{equation}
    \beta U_{Y}(r_{ij}^{*}) =
    \begin{cases}
        \frac{A}{r_{ij}^{*}}\left(e^{-r_{ij}^{*}/l_{c}} - e^{-r_{c}^{*}/l_{c}}\right), & \,\,\,\,r_{ij}^{*} \leq r_{c}^{*} \\
        0, & \,\,\,\,r_{ij}^{*} > r_{c}^{*}
    \end{cases}
    \label{eq:yukawa}
\end{equation}
where $A$ represents Yukawa coefficient, which is $a$ for cation-cation, $b$ for anion-anion, and $c$ for cation-anion. $l_{c}$ is the length of the Yukawa potential.

To investigate the effect of asymmetric Yukawa potential, the correlation strength between cation-cation, $a$, is fixed to 0.75 and $b$ and $c$ are varied within certain ranges: $0.1a\leq b \leq 1.4a$ and $0.9a\leq c \leq 1.2a$. And the cutoff distance is set to $r_{c}=L_{x}/2$. Hereinafter, fractions multiplied by the anion-anion coefficient and the cation-anion coefficient will be referred to as $\alpha_{b}$ and $\alpha_{c}$, respectively. Details of rest of pair potentials are explained in the section B of Supporting Information

Subsequently, simulations with uniform electric field are performed to elucidate the effect of asymmetric Yukawa interaction on the formation of crowding structure. Electric fields with strength $-1 \leq E \leq 1$ are applied to model potential differences with strength $-118 \leq\Delta V/V_{T}\leq 118$. For here, $V_{T}=k_{B}T/e \approx 11$ is the thermal voltage in LJ units and $\alpha$, and $\alpha_{c}$ are fixed to 0.75 and 1.1, while $\alpha_{b}$ being varied.


==> texFiles/03_results.tex <==
\section{Results}
\subsection{Statistical Field Theory}
When the short-range interaction is symmetric, \textit{i.e.} $a=b$, Eq.~\ref{eq:mf} yields,
\begin{equation}
\begin{split}
\frac{\nu}{4\pi l_{B}}\nabla^{2}\psi_{e} &= \tanh\left(\psi_{e} + \psi_{h}\right) \\
\frac{\nu}{2\pi(c-a)}\left(\nabla^{2}-\kappa^{2}\right)\psi_{h} &= \tanh\left(\psi_{e}+\psi_{h}\right),
\end{split}\label{eq:aeqb}
\end{equation}
where $\psi_{h} = -\psi_{2}/\sqrt{2}$. For this special case, our Eq.~\ref{eq:aeqb} is identical to the equations in previous work~\cite{bossa}. To check correspondences, we used boundary conditions~\cite{bossa, charge_oscillation}
\begin{equation}
\begin{split}
    \psi_{e}'(0) &= -\lambda s_{e} \\ \\
\begin{pmatrix} \psi_{1}'(0) - \kappa \psi_{1}(0) \\ \\ \psi_{2}'(0) - \kappa \psi_{2}(0) \end{pmatrix}
&= -4\pi A_{h}\begin{pmatrix} \sigma_{1} \\ \\ \sigma_{2}\end{pmatrix},
\end{split}\label{eq:bc}
\end{equation}
where $\lambda^{2}=4\pi l_{B}/\nu$ and $s_{e} = \lambda\sigma_{e}/e$. We set $\sigma_{1}=\sigma_{2}=0$ for the simplicity. We numerically solved these nonlinear differential equations and calculated dimensionless differential capacitance $\tilde{C}_{diff}=ds_{e}/d\psi_{0}$. Fig.~\ref{fig:ref_matching} shows our results match the previous results ~\cite{bossa} very well.

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Fig01a.eps}
         \label{fig:fig02a}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Fig01b.eps}
         \label{fig:fig02b}
     \end{subfigure}
    %\includegraphics[width=0.5\textwidth]{figures/Fig02.eps}
    \caption{\textbf{a.} Scaled surface charge density (dotted) and scaled differential capacitance (solid) as a function of surface electrostatic potential by varying $\alpha_{b}$ values, \textbf{b.} Scaled surface charge density as a function of $\alpha_{b}$; \footnotesize{$\alpha_{b}$ varies from 0.1 (most right) to 1.3 (most left) with an increment of 0.2 , and red markers show $s_{e}$ at $\psi_{0}$ where $\tilde{C}_{diff}$ diverges. If $s_{e}$ shows different values at certain $\psi_{0}$, there is charge separation at the $\alpha_{b}$.}}
    \label{fig:fig2}
\end{figure}

We explore the asymmetric case, which would be more adequate for real systems, $a \neq b$. We vary $b$ with fractions of $\alpha_{b}$. For instance, $b=a \times \alpha_{b}$, while fixing $a$ and $c$. We find numerical solutions of Eq.~\ref{eq:mf} under the boundary condition of  $\sigma_{1}=\sigma_{2}=0$. As shown in Fig.~\ref{fig:fig2}.a, unlike symmetric case, the $\psi_{0}-s_{e}$ curves deviates from $\psi_{0}=0$. Moreover, the $\psi_{0}-s_{e}$ curve shows hysteresis when there are charge separations, and they form a charged layer in the vicinity of the charged surface called the electric double layer (EDL). We calculated $\tilde{C}_{diff}=\frac{1}{d \psi_{0}/d s_{e}}$. As shown in Fig.~\ref{fig:fig2}.a, $\tilde{C}_{diff}$ becomes diverging when there is hysteresis in the $\psi_{0}-s_{e}$ curve. In other words, the system undergoes first-order transition when forming EDLs~\cite{bossa, charge_oscillation}. We found $\psi_{0}$ where $\tilde{C}_{diff}$ diverges and investigated the behavior of scaled surface charge density $s_{e}$. If $\tilde{C}_{diff}$ does not show divergence, cations and anions are homogeneously mixed in the system showing no charge separations. If $\tilde{C}_{diff}$ diverges, charge separations start to appear forming EDLs. At $\psi_{0}$ where $\tilde{C}_{diff}$ diverges, ions start to make structure such as oversereening or crowding. We will investigate the changes of ion structure at the onset of charge separations in the discussion section.

We varied the cation-anion interaction parameter $c$. We found that the onset of $\tilde{C}_{diff}$ divergence shifts toward lower $\alpha_{b}$ when increasing $c$ as shown in Fig.~\ref{fig:fig2}.b. Increasing the cation-anion interaction parameter $c$ enhances the short-range repulsive interaction between cations and anions, making ions easily aggregate due to the increased short-range repulsion between opposite charges. This may give the advantage to like charge forming layers near the charged surface at the lower $\alpha_{b}$ called EDLs.

\subsection{Molecular Dynamics Simulation}
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Fig02a.eps}
         \label{fig:fig03a}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/Fig02b.eps}
         \label{fig:fig03b}
     \end{subfigure}
    \caption{MD simulation results of Charge separation and differential capacitance; \footnotesize{As shown in Fig.~\ref{fig:charge_separation}.a, the surface charge density fluctuate around $0$, which denotes no charge separation at $c=0.9$. Charge separation occurs above $c=1.0$. When $c$ value increases, the onset of charge separation shift toward smaller $\alpha_{b}$, which show correspondence with field theoretic work.}}
    \label{fig:charge_separation}
\end{figure}

We performed MD simulations to validate our statistical field theoretic results. As we did in field theoretic analysis, we explored a range of Yukawa interaction parameters. We first calculated the local charge density profile $\rho_{c}(x)$ to quantify charge separation
\begin{equation}
\begin{split}
    \rho_{c}(x) = q\left(\langle n_{+}(x) \rangle - \langle n_{-}(x) \rangle \right),
\end{split}
\end{equation}
where the bracket denotes the ensemble average, and $n_{+}(x)$ and $n_{-}(x)$ are the number density profiles of cations and anions, respectively. The number density profiles are averaged over $y$ and $z$ axis and determined by dividing the real systems along the $x$-axis, examining the number of relevant ions within each interval, and subsequently normalizing the counts by the corresponding bin volumes. Then, the surface charge density $\sigma_{e}$ is obtained by 
\begin{equation}
s_{e} = \frac{\epsilon_{r} \Delta V}{4 \pi L_{x}} - \frac{1}{L_{x}}\int_{0}^{L_{x}} x \rho_{c}(x) dx,
\end{equation}
where $\Delta V$ is the difference of constant potential between electrodes. 

With zero-field simulations, we could see the effect of Yukawa potentials on the formation of EDLs in the absence of external field. As shown in Fig.~\ref{fig:charge_separation}.a, there is no charge separation at $\alpha_{c}=0.9$, where $\alpha_{c}=c/a$. From $\alpha_{c}=1.0$, charge separations start to appear. In addition, the onset of charge separation shifts toward a smaller $\alpha_{b}$ as $\alpha_{c}$ increases. The detailed discussion of these molecular mechanisms will be provided in the discussion section. This is analogous to our field-theoretic results shown in Fig.~\ref{fig:fig2}.b, showing the onset of charge separation shifts toward a lower $\alpha_{b}$ when increasing $\alpha_{c}$. However, with zero-field, crowding structure of EDLs was not observed through the all ranges of Yukawa coefficients we explored. From the ref~\cite{benjamine}, crwoding structure would be found when the values of $\alpha_{c}$ becomes huge. However, those of $\alpha_{c}$ are unphysical, making vaccum in the system. So, we used a proper values of $\alpha_{c}$, which is not showing crowding structure.

With applied potential differences, crowding structure of EDLs was observed within the wide range of the strength of electric field. As shown in Fig.~\ref{fig:ext_field_charge_density}, charge density profile of crowding structure emerges from certain values of applied potential differences while that of overscreening is observed with zero-field. From this result, we could speculate the phase transition to crowding is voltage-induced phase transition. 

To summarize MD results, we also validated the results in ref~\cite{bsk, kornyshev_md}, showing the dependence of external field in forming overscreening and crowding structure near the electrode. However, even without an external field, EDL structures such as overscreening are formed, and when the strength of yukawa interaction is asymmetric, charge separation, that is, the onset if EDL formation, is consistent with field theoretic research.

\begin{figure}%[htbp]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/Fig03.eps}
    \caption{Charge density profiles with and without external fields}
    \label{fig:ext_field_charge_density}
\end{figure}

\subsection{Limiting Case}
\underline{Case1}: If $a=b=c$, then $\theta=\pi/4$, $\lambda_1=a+c, \lambda_2=a-c$, and $\tilde{e_1}=\exp\left(-\psi_e+\frac{1}{\sqrt{2}}\left\{-\psi_1+\psi_2\right\}\right)$ and $\tilde{e_2}=\exp\left(\psi_e-\frac{1}{\sqrt{2}}\left\{-\psi_1 -\psi_2\right\}\right)$. 

==> texFiles/04_discussion.tex <==
\section{Discussion}
Pure electrostatic systems require a surface charge density much larger $1e/nm^2$ or existence of multivalent counter-ions to form EDL. 
Given that the EDL is formed even at very low voltage for ionic liquid, an additional mechanism enhancing counterion condensation is required. 
Since the IL consists of large delocalized charges, multipolar interactions, and hardcore exclusion would affect the charge correlations. 
In our model, other than monopolar charge interactions are incorporated in the Yukawa interactions. The effective short-range interaction is related to $\xi = a\left(1+\alpha_b-2\alpha_c\right)$. In the limit that the Yukawa term is negligible, for example, $\kappa=\infty$, $\phi_1$ and $\phi_2$ are zero; hence, the system will follow the pure electrostatic case. 
A negative value of $\xi$ enhances the demixing of two charged components, at least at the surfaces. 
If $\xi$ grows to a meaningful value, the simulation shows the formation of a condensation layer even in very low surface charge density. 
At the beginning of the simulation, two charges form local domains at both electrodes, which may be metastable due to large line tensions~\cite{benjamine}. 
Given enough time, the metastable state transits to a stable state, in which a single charge species is abundant in each electrode~\cite{benjamine, atkin}. The condensed layer easily overscreens the surface charges, which is extremely difficult to achieve for pure electrostatic cases. 

In our case, because the Yukawa coefficients adjusts the electrostatic interactions also, $\xi$ does not explain the surface phase demixing by itself. For example, increasing $a$ or $b$ differs from decreasing $c$ for the same $\xi$ because they also affect the Coulombic interactions. Smaller $\alpha_b$ makes the large anionic domain formation difficult, while increasing $c$ enhances it. 
If $\alpha_c$ is unreasonably large to ignore the Coulomb interaction, there would be a bulk phase transition due to the binary demixing. 

As seen in Fig.~\ref{fig:ext_field_charge_density}, a multiple-charged layer is formed by the voltage-induced transition within the parameter range we used.
The onset voltage for crowding depends on the effective and Coulomb interactions. Stronger short-range repulsion between opposite charges or attraction between like charges reduces the onset voltage~Fig.~\ref{fig:crowding_threshold}. Indeed, EDL formation, overscreening and crowding are all dependent on the shape of ionic liquid (or the strength of the short-range interaction) as well as the external electric field.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/Fig04.eps}
    \caption{Local charge density profiles calculated from the field theoretic results; \footnotesize{Local charge density profiles were calculated at the onset of the divergence of $\tilde{C}_{diff}$ as shown in Fig.~\ref{fig:fig2}.b.}}
    \label{fig:local_charge_density}
\end{figure}

The internal structure of EDLs, when the $\tilde{C}_{diff}$ diverges, also depends on the short-range interaction. We investigate local charge density profiles at the onset of divergence of $\tilde{C}_{diff}$ from our field-theoretic model. 
The average number of ions is  
\begin{equation}
    N_{\pm} = \lambda_{\pm}\frac{\partial \ln{\mathcal{Z}_{\lambda}}}{\partial \lambda_{\pm}}.
\end{equation}
The local charge density profile is obtained from the loop expansion adopted the zeroth order,
\begin{equation}
    \rho_{c}(r) = \sum_{i=\pm} \frac{N_{i}}{V} = \left\langle \frac{\tilde{e}_{1} - \tilde{e}_{2}}{\tilde{e}_{1} + \tilde{e}_{2}} \right\rangle = \frac{\bar{e}_{1} - \bar{e}_{2}}{\bar{e}_{1} + \bar{e}_{2}},
\end{equation}
where the potential in $\bar{e}_{1,2}$ is used as saddle-point solutions of $\psi_{e}, \psi_{1}$, and $\psi_{2}$. From the local charge density profiles in Fig.~\ref{fig:local_charge_density}, we find that condensed counterions underscreen the surface charge at $c \geq 1.742$. They start to
overscreen the surface charge at $1.342 \leq c \leq 1.642$. It is plausible that large repulsion between different species may induce EDL even at low surface charges, and hence below the overscreening condition. 

Previous studies have reported that IL EDL appears as overscreening or crowding depending on the surface charge density~\cite{Kornyshev, nmat}. However, they did not mention the ion structure of EDL at the onset of $\tilde{C}_{diff}$ divergnece. At the onset of divergence, we found the ion structures were not determined by single ion structure of EDL such as overscreening or crowding. %As shown in Fig.~\ref{fig:local_charge_density}, ion packing structures become sparse as an increase of short-range cation-anion interactions.

Based on our results, we carefully think that explicit consideration of ion-ion interactions such as short-ranged, long-ranged ion-ion correlations, and ion size, we, again, carefully suggest that the structure of EDLs is affected by the strength of short-ranged cation-anion interactions. So, the structures of EDLs might depend on the system conditions. As shown in the BSK model, if the short-range ion interaction becomes strong, the structure of EDLs is observed as crowding, which is validating our model, as shown in S.I~\cite{bsk}.


==> texFiles/05_conclusion.tex <==
\section{Conclusion}
In this study, we incorporate Coulomb and Yukawa interaction potential within the framework of the statistical field theory. We demonstrate that EDL for ionic liquid is formed from two cooperating mechanisms: a strong coupling of electrostatic interaction and phase demixing due to the short-range interaction. The first mechanism requires high surface charge density and the presence of multivalent counterions for overscreening or crowding. On the other hand, the second mechanism may induce condensation layer even at low surface charge density. 
The divergence of differential capacitance at low external field points out that the short-range interaction due to IL's large delocalized charges. 

The structure of EDLs at the onset of divergence of $\tilde{C}_{diff}$ does not appear to be single structure. It depends on the system conditions, such as the strength of short-ranged ion-ion correlations and surface charge density. Considering these ionic liquids' properties, we can apply these results to real-world problems such as supercapacitors and solid-state electrolytes modeling. Through healthy discussions, we eagerly await the evolution of understanding in ionic liquids.

\renewcommand\thesection{}
\section{Author Contribution}
This section is intentionally left empty.

\section{Data Availability}
The authors will provide data on reasonable request. 

\section{Acknowledgement}
This research was supported by the National Research Foundation of Korea(NRF) grant funded by the Korea government(MSIT) 2018M3D1A1058624, and 2021R1A2C1014562.
